A Bayesian approach for consistent reconstruction of inclusions

This paper considers a Bayesian approach for inclusion detection in nonlinear inverse problems using two known and popular push-forward prior distributions: the star-shaped and level set prior distributions. We analyze the convergence of the corresponding posterior distributions in a small measurement noise limit. The methodology is general; it works for priors arising from any H\"older continuous transformation of Gaussian random fields and is applicable to a range of inverse problems. The level set and star-shaped prior distributions are examples of push-forward priors under H\"older continuous transformations that take advantage of the structure of inclusion detection problems. We show that the corresponding posterior mean converges to the ground truth in a proper probabilistic sense. Numerical tests on a two-dimensional quantitative photoacoustic tomography problem showcase the approach. The results highlight the convergence properties of the posterior distributions and the ability of the methodology to detect inclusions with sufficiently regular boundaries.

==> figures/tikz-spaces.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,463); %set diagram left start at 0, and has height of 463

%Curve Lines [id:da6919578609090795] 
\draw    (155.67,158.67) .. controls (193.69,136.24) and (318.99,157.62) .. (354.76,172.38) ;
\draw [shift={(357.33,173.5)}, rotate = 203.31] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- cycle    ;
%Shape: Rectangle [id:dp6325359567456931] 
\draw   (93.67,129) -- (220.33,129) -- (220.33,250) -- (93.67,250) -- cycle ;
%Curve Lines [id:da5885533016953061] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (293.33,236.83) .. controls (360.33,194.83) and (268.98,171.98) .. (290.98,150.98) .. controls (315.98,125.98) and (362.98,136.98) .. (359.98,177.98) .. controls (357.31,219.48) and (360.65,236.15) .. (383.65,236.15) ;
%Curve Lines [id:da19735346376906182] 
\draw    (175,230.67) .. controls (196.07,203.96) and (272.23,193.74) .. (313.2,202.76) ;
\draw [shift={(315.67,203.33)}, rotate = 192.41] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- cycle    ;
%Curve Lines [id:da8737072060510577] 
\draw    (142.33,196) .. controls (188.07,175.75) and (271.92,192.63) .. (313.19,202.72) ;
\draw [shift={(315.67,203.33)}, rotate = 193.79] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- cycle    ;
%Shape: Circle [id:dp9590690681983736] 
\draw  [draw opacity=0][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (137.84,197) .. controls (137.84,195.44) and (139.11,194.18) .. (140.67,194.18) .. controls (142.23,194.18) and (143.49,195.44) .. (143.49,197) .. controls (143.49,198.56) and (142.23,199.82) .. (140.67,199.82) .. controls (139.11,199.82) and (137.84,198.56) .. (137.84,197) -- cycle ;
%Shape: Rectangle [id:dp5405568525453104] 
\draw   (270.33,129) -- (397,129) -- (397,250) -- (270.33,250) -- cycle ;
%Shape: Circle [id:dp2196102447930519] 
\draw  [draw opacity=0][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (172.18,230.67) .. controls (172.18,229.11) and (173.44,227.84) .. (175,227.84) .. controls (176.56,227.84) and (177.82,229.11) .. (177.82,230.67) .. controls (177.82,232.23) and (176.56,233.49) .. (175,233.49) .. controls (173.44,233.49) and (172.18,232.23) .. (172.18,230.67) -- cycle ;
%Shape: Circle [id:dp9214840221039564] 
\draw  [draw opacity=0][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (152.84,158.67) .. controls (152.84,157.11) and (154.11,155.84) .. (155.67,155.84) .. controls (157.23,155.84) and (158.49,157.11) .. (158.49,158.67) .. controls (158.49,160.23) and (157.23,161.49) .. (155.67,161.49) .. controls (154.11,161.49) and (152.84,160.23) .. (152.84,158.67) -- cycle ;
%Shape: Circle [id:dp3732969079565861] 
\draw  [draw opacity=0][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (315.67,204.33) .. controls (315.67,202.77) and (316.93,201.51) .. (318.49,201.51) .. controls (320.05,201.51) and (321.31,202.77) .. (321.31,204.33) .. controls (321.31,205.89) and (320.05,207.16) .. (318.49,207.16) .. controls (316.93,207.16) and (315.67,205.89) .. (315.67,204.33) -- cycle ;
%Shape: Circle [id:dp727516649832411] 
\draw  [draw opacity=0][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (357.16,174.16) .. controls (357.16,172.6) and (358.42,171.33) .. (359.98,171.33) .. controls (361.54,171.33) and (362.8,172.6) .. (362.8,174.16) .. controls (362.8,175.71) and (361.54,176.98) .. (359.98,176.98) .. controls (358.42,176.98) and (357.16,175.71) .. (357.16,174.16) -- cycle ;

% Text Node
\draw (101,133.4) node [anchor=north west][inner sep=0.75pt]    {\Large $\Theta $};
% Text Node
\draw (355,133.4) node [anchor=north west][inner sep=0.75pt]    {\small $L^2_\Lambda(D) $};
% Text Node
\draw (368.33,207.23) node [anchor=north west][inner sep=0.75pt]    {\Large $\Gamma $};
% Text Node
\draw (326,196.09) node [anchor=north west][inner sep=0.75pt]    {\Large $\gamma $};
% Text Node
\draw (155,226.42) node [anchor=north west][inner sep=0.75pt]    {\Large $\theta $};
% Text Node
\draw (241,208) node [anchor=north west][inner sep=0.75pt]    {\Large $\Phi $};


\end{tikzpicture}


==> old-files/Lemma-on-tests.tex <==

\begin{lemma}
    Suppose Condition \ref{cond:non-uniform} is satisfied. Then there exists a measurable function $\Psi_\varepsilon:\mathcal{Y}_{-}\rightarrow \{0,1\}$ such that Condition \ref{cond:1}.\ref{cond:1.3} is satisfied for 
    \begin{equation}\label{eq:bad-a-rate}
        a > \frac{1}{1+t\tau/2}.
    \end{equation}
\end{lemma}
\begin{proof}
    See \cite[Lemma 8]{abraham2019}. Define first the estimator $\hat{\mathcal{G}}:\mathcal{Y}_{-}\rightarrow \mathcal{Y}_{-}$,
    $$\hat{\mathcal{G}}(y) = \sum_{n=1}^{N} y_n e_n =: P_n y,$$
    for $N=N_\varepsilon = \lfloor \frac{r_\varepsilon}{\varepsilon} \rfloor$.
    We will show that 
    $$\Psi_\varepsilon(y) := \mathds{1}_{\|\hat{\mathcal{G}}(y) - \mathcal{G}(\gamma_0)\|>\frac{1}{2}C_0 r_\varepsilon}$$
    is good enough.  First, by the triangle inequality,
    \begin{align}\label{eq:bias-variance}
        P_\varepsilon^\gamma(\|\hat{\mathcal{G}}(Y)&-\mathcal{G}(\gamma)\|>C'r_\varepsilon) \leq \\ &P_\varepsilon^\gamma(\|\hat{\mathcal{G}}(Y)-P_N\mathcal{G}(\gamma)\|>\frac{1}{2}C'r_\varepsilon) + \mathds{1}_{\|P_N\mathcal{G}(\gamma)-\mathcal{G}(\gamma)\|>\frac{1}{2}C'r_\varepsilon}.
    \end{align}
    By the last part of Condition \ref{cond:non-uniform} for all $\gamma \in \Gamma'$ and for $\gamma=\gamma_0$
    \begin{align}
        \|P_N\mathcal{G}(\gamma)-\mathcal{G}(\gamma)\|^2 \leq \lambda_{N+1}^{t} \|\mathcal{G}(\gamma)\|_{t}^2 \leq M N^{-t\tau}.
    \end{align}
    The second term in \eqref{eq:bias-variance} then vanishes if $N^{-t\tau/2}$ decays faster than $r_\varepsilon$, which is exactly when $a$ satisfies \ref{eq:bad-a-rate}. As argued in \cite{abraham2019} the first term in \eqref{eq:bias-variance} satisfies for any $\kappa>0$ and $C'$ large enough depending on $\kappa$
    $$P_\varepsilon^\gamma(\|\hat{\mathcal{G}}(Y)-P_N\mathcal{G}(\gamma)\|>\frac{1}{2}C'r_\varepsilon)\leq e^{-\kappa (r_\varepsilon/\varepsilon)^2}.$$
    Then taking $\gamma=\gamma_0$ and setting $C_0=2C'$, a direct consequence of \eqref{eq:bias-variance} is
	$$E_\varepsilon^{\gamma_0}(\Psi_{\varepsilon})=P_\varepsilon^{\gamma_0}(\|\hat{\mathcal{G}}(Y)-\mathcal{G}(\gamma_0)\|>\frac{1}{2}C_0r_\varepsilon) \leq e^{-\kappa(r_\varepsilon/\varepsilon)^2}$$
	Also by the triangle inequality, 
	\begin{align}
		E_\varepsilon^{\gamma}(1-\Psi_{\varepsilon}) &= P_{\varepsilon}^{\gamma} (\|\hat{\mathcal{G}}(Y)-\mathcal{G}(\gamma_0)\|\leq \frac{1}{2}C_0r_\varepsilon ),\\
		&\leq P_{\varepsilon}^{\gamma} (-\|\hat{\mathcal{G}}(Y)-\mathcal{G}(\gamma)\| + \|\mathcal{G}(\gamma)-\mathcal{G}(\gamma_0)\| \leq \frac{1}{2}C_0r_\varepsilon ),\\
		&\leq P_{\varepsilon}^{\gamma} ( \|\hat{\mathcal{G}}(Y)-\mathcal{G}(\gamma)\| \geq \|\mathcal{G}(\gamma)-\mathcal{G}(\gamma_0)\|-\frac{1}{2}C_0r_\varepsilon ),
	\end{align}
	where taking $\sup_{\gamma\in \Gamma' : d_{\mathcal{G}}(\gamma_0,\gamma)>C_0r_\varepsilon }$ on both sides of the inequality gives the wanted property.
\end{proof}

\begin{theorem}\label{thm:3.6}
    Suppose the conditions of Theorem 3.5 with Condition \ref{cond:unifcont} replaced by \ref{cond:non-uniform} is satisfied. Then
    $$\Pi(\gamma:\|\gamma-\gamma_0\|_{L^2(D)}\leq f(C_0r_\varepsilon)|Y)\rightarrow 1 \quad \text{ in $P_{\varepsilon}^{\gamma_0}$-probability},$$
    where $r_\varepsilon=\varepsilon^{1-a}$ with
    $$a>\max\left\{\frac{n}{2\eta\zeta \beta + n},\frac{1}{1+t\tau/2}\right\}.$$
\end{theorem}

==> old-files/level-set.tex <==
For simplicity we assume $f(x) = x^\nu$ for some $0<\nu<1$. Then we shall see in the proof of Theorem \eqref{eq:level-set-const} below, taking
$$\delta = \varepsilon^k$$
for some well-chosen $0<k<1$ balances the contraction rate of the posterior distribution around $\gamma_0^\varepsilon$ with the convergence rate of $\gamma_0^\varepsilon$ to $\gamma_0$.

\begin{theorem}\label{eq:level-set-const}
    Let $\Gamma = \Phi(H^{\alpha}(D))$, $\alpha>1+n/2$ and suppose Condition \ref{cond:forward-map} is satisfied for $\Theta'$ in \eqref{eq:Thetaprimelevel}. Define $\Pi$ as above for $\beta>2+n/2$ and let 
    $$\gamma_0 = \Phi(\theta_0),$$
    $\theta_0\in \mathcal{H}$. If $\Pi(\cdot|Y)$ is the corresponding sequence of posterior distributions arising for the model \eqref{eq:obs}. Then
    $$\Pi(\gamma:\|\gamma-\gamma_0\|_{L^2(D)}\leq C_0r_\varepsilon^\nu |Y)\rightarrow 1 \quad \text{ in $P_n^{\gamma_0}$-probability},$$
    where $r_\varepsilon=\varepsilon^{1-a}$ with
    \begin{equation}\label{eq:final-cond-on-a-level}
            a \geq \frac{2\eta\nu d+ d}{2\eta\nu d + 2\delta\eta + d}.
    \end{equation}
    \begin{proof}
    % triangle inequality argument
    % contraction around gamma_0^\varepsilon
    For any $\tilde{r}_\varepsilon>0$, the triangle inequality yields
    $$\left\{\gamma: \|\gamma-\gamma_0\|_{L^2(D)}\leq C_0\tilde{r}_\varepsilon\right\}\supset \left\{\gamma: \|\gamma-\gamma_0^\varepsilon\|_{L^2(D)}\leq \frac{1}{2}C_0\tilde{r}_\varepsilon, \|\gamma_0^\varepsilon-\gamma_0\|_{L^2(D)}\leq \frac{1}{2}C_0\tilde{r}_\varepsilon\right\},$$
    hence
    \begin{align}
        \Pi(\gamma:\|\gamma-\gamma_0\|_{L^2(D)}\leq C_0\tilde{r}_\varepsilon |Y) &\geq \Pi(\gamma:\|\gamma-\gamma_0^\varepsilon\|_{L^2(D)}\leq \frac{1}{2}C_0\tilde{r}_\varepsilon|Y)\\
        &\times \mathds{1}_{\|\gamma_0^\varepsilon-\gamma_0\|_{L^2(D)}\leq \frac{1}{2}C_0\tilde{r}_\varepsilon}. \label{eq:triangle-argument}
    \end{align}
    We shall consider the two factors of the right-hand side in separate parts below:

    \noindent 1) We check that conditions \ref{cond:1}.\ref{cond:1.1}, \ref{cond:1}.\ref{cond:1.2}, and \ref{cond:1}.\ref{cond:1.3} are satisfied. Starting with \ref{cond:1}.\ref{cond:1.1} we proceed as in the proof of Lemma \ref{lemma:small-ball} and use Lemma \ref{lemma:4.5} to obtain
    \begin{align}
		\{\theta \in \Theta: d_{\mathcal{G}}(\Phi_{\varepsilon^k}(\theta),&\Phi_{\varepsilon^k}(\theta_0))\leq r_{\varepsilon}\}\\
			&\supset \{\theta\in \Theta: \|\theta-\theta_0\|_{L^\infty(D)} \leq C\varepsilon^k r_{\varepsilon}^{\frac{1}{\eta}}, \|\theta-\theta_0\|_{H^{\beta}(\mathcal{X})}\leq \tilde M\}, 
		\end{align}
		where $C=C(\eta,\zeta,C_{\mathcal{G}},C_{\Phi})$. Continuing the argument, it suffices to have
        $$(r_\varepsilon^{\frac{1}{\eta}}\varepsilon^{k-a})^{-b}\leq (r_\varepsilon/\varepsilon)^2,$$
        for $b=\frac{2d}{2\delta-d}$. This is satisfied for the choice 
    \begin{equation}\label{eq:cond-on-a}
            a \geq \frac{d(\eta k+1)}{2\delta\eta+d},
    \end{equation}
    where we also note that $k$ should satisfy
        \begin{equation}\label{eq:on-k}
            0<k<\frac{2\delta}{d},
        \end{equation}
        so that $0<a<1$. Next, to satisfy condition \ref{cond:1}.\ref{cond:1.2} we need to satisfy
    \begin{equation}\label{eq:prior-cond-level}
        \Pi(L^2_\Lambda(D)\setminus \Gamma'_\varepsilon) = \Pi'(\Phi^{-1}_{\varepsilon^k}(L^2_\Lambda(D)\setminus \Gamma'_\varepsilon)) = \Pi'(H^\alpha(D)\setminus \Theta_\varepsilon') \leq e^{-C_2(r_\varepsilon/\varepsilon)^2},
    \end{equation}
    with $C_2>C_1+2$ for some $C_1>0$. Under our assumptions $\theta \sim \Pi'$ is almost surely in $C^1(D)$ and $(\theta(x):x\in D)$ is a centered stationary Gaussian process. Then, $(\theta(x),\partial_1\theta(x),\hdots,\partial_2\theta(x))$ is a centered Gaussian vector with a constant non-degenerate covariance matrix (dependent on $\varepsilon$) for each $x\in D$, see for example Exercise 6.2 \cite{azais2009}. Then by \cite[Proposition 6.12]{azais2009}
        $$\Pi'(H^\beta_\diamond(D)) = 1,$$
        for each $\varepsilon>0$. Since 
        $$H^\alpha(D)\setminus \Theta'_\varepsilon = (H^\alpha(D) \cap \Theta_\varepsilon) \cup (H^\alpha(D) \cap H^\beta_\diamond(M)^c),$$
        it follows that
        $$\Pi'(H^\alpha(D)\setminus \Theta'_\varepsilon)\leq \Pi'(H^\alpha(D)\setminus \Theta_\varepsilon),$$
        and hence \eqref{eq:prior-cond-level} is satisfied by Lemma .
        Condition \ref{cond:1.3} is satisfied as in lemma \ref{lemma:3.3} using that $\Theta_\varepsilon'\subset \Theta_\varepsilon$. By the properties of $\mathcal{G}$ and $\Phi_{\varepsilon^k}$ we have for any $\rho>0$
         $$ \log N(\Gamma'_\varepsilon, d_\mathcal{G}, C\varepsilon^{-k\eta}\rho^{\eta}) \leq \log N(\Theta_\varepsilon', \|\cdot\|_{L^\infty(\mathcal{X})}, \rho) \leq C\rho^{-d/\delta}. $$
         Then for all $\varepsilon >0$
\begin{align}
    \log N(\{\gamma \in \Gamma'_\varepsilon: r_\varepsilon < d_{\mathcal{G}}(\gamma,\gamma_0)<2r_\varepsilon\},d_{\mathcal{G}},r_\varepsilon)&\leq C(r_\varepsilon \varepsilon^{k\eta})^{-\frac{d}{\delta \eta}},\\
   &< C(r_\varepsilon/\varepsilon)^2,
\end{align}
for the choice \eqref{eq:cond-on-a}, hence condition \ref{cond:1.3} is satisfied. Then by Theorem \ref{thm:contr}
$$\Pi(B_{\mathcal{G}}(\gamma_0^\varepsilon,Cr_\varepsilon) \cap \Gamma'_\varepsilon | Y) \rightarrow 1 \quad \text{ in $P_n^{\gamma_0}$-probability},
$$
    as $\varepsilon \rightarrow 0$ for some constant $C>0$. Then by condition \ref{cond:forward-map} and \eqref{eq:inv-stability-cont}
$$\Pi(\|\gamma-\gamma_0^\varepsilon\|_{L^2(D)} \leq C_0'r_\varepsilon^\nu | Y) \rightarrow 1 \quad \text{ in $P_n^{\gamma_0}$-probability},
$$
\noindent 2) For the second factor, note that lemma \ref{lemma:4.5} (i) implies
$$\|\gamma_0^\varepsilon-\gamma_0\|_{L^2(D)}\leq C(\theta_0)\varepsilon^{k/2}.$$
Since $r_\varepsilon^\nu$ is a strictly growing function of $k$ (the rate becomes worse for larger $k$) and $\varepsilon^{k/2}$ is strictly decreasing in $k$, the optimal choice of $k$ satisfies
$$r_\varepsilon^\nu = \varepsilon^{k/2}.$$
This is solved by
    \begin{equation}\label{eq:cond-on-k}
        k = \frac{2\delta}{d+\frac{\delta}{\nu}+\frac{d}{2\nu\eta}},
    \end{equation}
which also satisfy \eqref{eq:on-k}. Inserting this back into \eqref{eq:cond-on-a} yields \eqref{eq:final-cond-on-a-level}. Finally, take $C_0 = 2\max(C_0',C(\theta_0))$ and $\tilde{r}_\varepsilon = r_\varepsilon^\nu$ and note by \eqref{eq:triangle-argument} that
$$ \Pi(\gamma:\|\gamma-\gamma_0\|_{L^2(D)}\leq C_0 r_\varepsilon^\nu |Y) \geq \Pi(\gamma:\|\gamma-\gamma_0^\varepsilon\|_{L^2(D)}\leq \frac{1}{2}C_0r_\varepsilon^\nu|Y)\rightarrow 1,$$
in $P_n^{\gamma_0}$-probability.
\end{proof}
\end{theorem}
As expected we see that for weak inverse stability estimates, i.e. $\nu$ small, the obtained contraction rate approaches the usual rate \eqref{eq:contraction-rate-a}.


==> old-files/name.tex <==

\section{The level-set parametrization} \label{section:5} 
The main part of realizing Theorem \ref{thm:contr} for a certain $\Phi$ is constructing a set $\Theta'$ for which $\Phi$ is uniformly continuous and which is given enough mass by $\Pi'$ in the sense of Condition \ref{cond:1.2}. In this section we will give such a set $\Theta'$ for the well-known level-set parametrization on the form 
$$\Phi(\theta) = \sum_{i=1}^{\mathcal{N}} \rho_i \mathds{1}_{D_i(\theta)},$$
where $D_i(\theta)$ are subsets of $D$ parametrized by $\theta \in \Theta=H^\alpha(\mathcal{X})$ for $\alpha > 1+n/2$ and $\mathcal{X}=D$, see also Remark \ref{remarkonX}. To construct the level-set parametrization take constants $c=\{c_i\}_{i=1}^{\mathcal{N}}$ satisfying $-\infty = c_0 < c_1 <\hdots < c_\mathcal{N} = \infty$ for some $\mathcal{N}\in \mathbb{N}$. Given $\theta: \mathcal{X}\rightarrow \mathbb{R}$ define
$$D_i(\theta) :=\{x\in D: c_{i-1} \leq \theta(x) < c_i \}, \quad i=1,\hdots,\mathcal{N},$$
so that $\overline{D}=\cup_{i=1}^\mathcal{N} \overline{D}_i$ and $D_i \cap D_j = \emptyset$ for $i\neq j$. Constructing $\Theta'$ is made difficult by the fact that we in general have no uniform $C^1$ norm bound on the local graph representation of $\partial D_i(\theta)$ for $\theta \in C^1(\mathcal{X})$. This would require a lower bound on $|\nabla \theta|$ near $\{x\in \mathcal{X}:\theta(x) = c_i, i = 1,\hdots, \mathcal{N}\}$ as can be seen from the implicit function theorem. Instead, we should use the properties of $D_i(\theta)$ for Gaussian processes more directly. In fact, the expected geometric properties of so-called excursion sets $\{x \in \mathcal{X}: \theta(x) > u\}$ for stochastic processes are well-understood [Adler]. In the following we define
$$A_u(\theta) := \{x\in\mathcal{X}:\theta(x)>u \},$$
$$\sigma_u(\theta) := \{x\in\mathcal{X}:\theta(x)=u \},$$
and let $\lambda^{n-1}$ denote the $n-1$'th Lebesgue measure and let $|\cdot| = \lambda^n(\cdot)$ and $\lambda^0(\cdot)$ denote the counting measure.
\begin{lemma}\label{lemma:4.1}
Let $\Pi''$ be a centred Gaussian distribution on $H^\alpha(\mathcal{X})$, $\alpha > 1+n/2$. Suppose the Gaussian process $\{\theta(x): x\in \mathcal{X}\}$ is stationary for $\theta\sim \Pi''$, i.e. $\mathbb{E}[\theta(x)\theta(y)]=K(x-y)$ for some continuous function $K$. Then the following hold:
\begin{enumerate}[label=(\roman*)]
  \item For all $u\in \mathbb{R}$,
  \begin{equation}
      \mathbb{E}(|A_u(\theta)|)= |\mathcal{X}|(1-\Phi(u/K(0))),
  \end{equation}
  where $\Phi$ denotes the cumulative distribution function of a standard normal distribution.
  \item For all $u\in \mathbb{R}$, $|\sigma_u(\theta)|=0$ almost surely. Further, if $\theta \in C^2(\mathcal{X})$ almost surely and $K(0)>0$, then
  \begin{equation}
      \mathbb{E}(\lambda^{n-1}(\sigma_u(\theta))) = C|\mathcal{X}|\phi(u/K(0)),
  \end{equation}
  where $C$ is only dependent on $K$ and $\phi$ denotes the probability density function of a standard normal distribution.
\end{enumerate}
\end{lemma}
\begin{proof}
   $(i)$ By Fubini's theorem and stationarity,
   $$\mathbb{E}\left(\int_{\mathcal{X}} \mathds{1}_{A_u(\theta)}(x) \, dx \right) = \int_{\mathcal{X}} \mathrm{Pr}(\theta(x) > u) \, dx = |\mathcal{X}| (1-\Phi(u/K(0))).$$
   $(ii)$ It is straightforward to show $|\sigma_u(\theta)|=0$, see for example \cite{igelsias2016}. We use the Rice formula \cite[Theorem 6.8]{azais2009} and \cite[Proposition 6.12]{azais2009} in the stationary case 
   $$\mathbb{E}(\lambda^{n-1}(\sigma_u(\theta)))= \frac{1}{K(0)}\phi(u/K(0))\int_{\mathcal{X}} \mathbb{E}(|(\nabla \theta)(x)|)\, dx.$$
   It is straightforward to show that $(\nabla \theta)(x)$ is a centred Gaussian random vector with covariance $C:\mathbb{R}^n\rightarrow \mathbb{R}^n$, where $\mathrm{tr}(C) = -(\Delta K)(0)$. Using Jensen's inequality
   $$\mathbb{E}(|(\nabla\theta)(x)|)^2 \leq \mathbb{E}(|(\nabla\theta)(x)|^2) = \mathrm{tr}(C) = -(\Delta K)(0).$$
   It is a standard argument that $C^1$ path regularity implies that $K$ is twice continuously differentiable, see for example \cite[Section 1.4]{azais2009}. In the case $n=1$, we use the Rice formula for $\theta\in C^1(\mathcal{X})$, see \cite[Theorem 3.2]{azais2009}.
\end{proof}

It is well-known that $\Phi:C(\mathcal{X})\rightarrow L^p(D)$, $1<p<\infty$ is continuous \cite{igelsias2016}. To get a uniform Hölder constant we instead restrict ourselves to a subset of $\Theta$. This subset a common setting in for example density level set estimation \cite{rigollet2009}. In the following we use sets
$$V_{\delta,u}(\theta):=\{x\in \mathcal{X}:|\theta(x)-u|\leq \delta\},$$
$$V_{c}:=\{\theta\in \Theta: |V_{\delta,c_i}(\theta)| \leq \delta \text{ for each } i=1,\hdots,\mathcal{N}\}.$$
\begin{lemma}\label{lemma:4.2}
    For $\theta_1 \in V_c$, $\theta_2\in \Theta$, and $\|\theta_1-\theta_2\|_{L^\infty(\mathcal{X})}$ small enough,
    $$ \|\Phi(\theta_1)-\Phi(\theta_2)\|_{L^2(D)}\leq C\|\theta_1-\theta_2\|_{L^\infty(\mathcal{X})}^{1/2},$$
    for some constant $C=C(\mathcal{N})>0$.
\end{lemma}
\begin{proof}
    Let $\theta_\delta = \theta_2-\theta_1$ with $\|\theta_\delta\|_{L^\infty(\mathcal{X})} =: \delta$. As in \cite{igelsias2016} for $\delta$ small enough
   $$ \|\Phi(\theta_1)-\Phi(\theta_2)\|_{L^2(D)}^2 \leq \sum_{i=1}^{\mathcal{N}-1} |A_{i,\delta}| + \sum_{i=2}^{\mathcal{N}} |B_{i-1,\delta}|,$$
   where
   $$A_{i,\delta} = \{x\in \mathcal{X} : c_i \leq \theta_1(x) < c_i - \theta_\delta(x)\},$$
   $$B_{i-1,\delta} = \{x\in \mathcal{X} : c_{i-1}-\theta_\delta(x)\leq \theta_1(x) < c_{i-1}\}.$$
   Clearly, the condition $|V_{\delta,c_i}(\theta_1)|\leq \delta$ for $i=1,\hdots,\mathcal{N}$ is sufficient.
\end{proof}
An attractive property of the piecewise constant functions that arise from $C^1$ functions is that they have a $W^{s,p}$-Sobolev regularity exponent $s<1/p$. If we restrict ourselves to the subset of $\Theta$ of functions, for $n=1,2$, with uniformly bounded $\lambda^{n-1}$-area we can make a uniform bound on this Sobolev norm. Define
$$\sigma_c(M):=\{\theta\in \Theta: \lambda^{n-1}(\sigma_{c_i}(\theta)) \leq M \text{ for each } i=1,\hdots,\mathcal{N}\}$$
\begin{lemma}\label{lemma:4.3}
    If $n=1,2$ and $\theta\in \sigma_c(M)$, then
    $$\|\Phi(\theta)\|_{W^{s,p}(D)}\leq M',$$
    for all $1\leq p < \infty$, $s<1/p$, and where $M'>0$ is a constant only dependent on $M$, $n$, $s$, $p$, $\mathcal{X}$ and $\mathcal{N}$.
\end{lemma}
\begin{proof}
    By [Sickel99,Faraco13] we have
	$$\|\mathds{1}_{D_i(\theta)}\|_{W^{s,p}(\mathbb{R}^2)} \leq C(s,n,p,\mathcal{X}) \left (|D_i(\theta)|+\int_0^{\mathrm{diam}(\mathcal{X})} |(\partial D_i(\theta))_\delta| \frac{d \delta}{\delta^{1+ps}} \right)^{1/p}.$$
	Using Steiner's inequality [tubes, weyls paper] it holds 
    $$|(\partial D_i(\theta))_\delta|\leq 2\delta\left( \lambda^{n-1}(\sigma_{c_{i-1}}(\theta))+\lambda^{n-1}(\sigma_{c_i}(\theta))\right),$$
    since $\partial D_i(\theta) = \sigma_{c_{i-1}}(\theta)\cup \sigma_{c_{i}}(\theta)$. Then for $s<1/p$,
    \begin{align}
        \int_0^{\mathrm{diam}(\mathcal{X})} |(\partial D_i(\theta))|\frac{d \delta}{\delta^{1+ps}}&\leq  4MC(p,s,\mathcal{X}).
    \end{align}
    Using boundedness of the extension operator and the triangle inequality, we arrive at the wanted property.
\end{proof}
\begin{remark}\label{remarkonX}
    If instead $\mathcal{X}\supset D$ was a bounded connected domain in $\mathbb{R}^n$, and we defined
    $$D_i(\theta) :=\{x\in \mathcal{X}: c_{i-1} \leq \theta(x) < c_i \} \cap D, \quad i=1,\hdots,\mathcal{N},$$
    Lemma \ref{lemma:4.2} and \ref{lemma:4.3} still hold. 
\end{remark}
Note the surface area condition does not follow from a uniform bound on any regularity norm of $\theta$. As shown in [length of level set curves], the surface area of level sets has to do with curvature, which is not easy to bound in general. However, asymptotically, this condition is satisfied for samples of sufficiently regular Gaussian fields. 

\begin{lemma}\label{lemma:excess-mass-level}
    Define $\Theta' := \mathcal{S}_\beta(M)\cap V \cap \sigma(M')$ for sufficiently large $M$ and $M'$. Let $\Pi''$ be a Gaussian prior as defined in Section \ref{sec:gaussprior} for $\alpha>1+n/2$ and $\beta>2+n/2$ and such that $\{\theta''(x): x\in \mathcal{X}\}$ is stationary for $\theta''\sim \Pi''$. Then there exists levels $c$ such that $\Pi'$ defined by \eqref{eq:scaled-prior} satisfies for any given $C_2>0$
    $$\Pi'(\Theta\setminus\Theta')\leq e^{-C_2(r_\varepsilon/\varepsilon)^2},$$
   In fact, with a little tweaking $\min_{i=1,\hdots,\mathcal{N}} |c_i| > \|\theta_0\|_{\mathcal{H}}\geq \|\theta_0\|_{\infty}$.
   \textcolor{red}{This makes everything useless, as $\Phi(\theta_0)=\kappa_1$ for all such $\theta_0$. So hurray we can recover the constant function.}
\end{lemma}
\begin{proof}
    We show that $\Pi'(\Theta\setminus \Theta')\leq e^{-C_2(r_\varepsilon/\varepsilon)^2}$ by showing this property for $\mathcal{S}_\beta(M)^c$, $V^c$ and $\sigma(M')^c$ for a constant $\tilde{C_2}>C_2$. Then a union bound gives the result. The property for $\mathcal{S}_\beta(M)^c$ follows from Lemma \ref{lemma:3.1}. Next, we note
    $$|V_{\delta,c}(\theta)|=|\overline{A_{c-\delta}(\theta)}|-|A_{c+\delta}(\theta)|.$$
    By \ref{lemma:4.1} (i), and the fact that $|\sigma_{c-\delta}(\theta)|=0$ almost surely,
    \begin{align}
        \mathbb{E}(|V_{\delta,c}(\theta)|) &= |\mathcal{X}|\left(\Phi(\frac{c+\delta}{K(0)})-\Phi(\frac{c-\delta}{K(0)})\right),\\
        & \leq C\delta e^{-\frac{1}{2K(0)^2}c^2}.
    \end{align}
    By Markov's inequality,
    \begin{align}
        \Pi'(V^c) &= \sum_{i=1}^\mathcal{N}
        \Pi'(|V_{\delta,c_i}(\theta)|>\delta),\\
        &= \sum_{i=1}^\mathcal{N}\Pi''(|V_{\delta\varepsilon^{-a},c_i\varepsilon^{-a}}(\theta'')|>\delta),\\
        &\leq C\varepsilon^{-a}\sum_{i=1}^\mathcal{N} e^{-\frac{1}{2K(0)^2}(c_i\varepsilon^{-a})^2},\\
        &\leq e^{-\tilde{C_2}(r_\varepsilon/\varepsilon)^2},
    \end{align}
    for $\min_{i=1,\hdots,\mathcal{N}} c_i^2 > 2\tilde{C_2}K(0)^2$ and $\varepsilon$ small enough. The same property for $\sigma(M')$ follows from Lemma \ref{lemma:4.1} (ii) by a similar argument.
\end{proof}

\begin{theorem}
    Let $\Phi$ and $\Pi'$ be as in Lemma \ref{lemma:excess-mass-level} for $\alpha>1+n/2$ and $\beta>2+n/2$. Let $\gamma_0=\Phi(\theta_0)$ for $\theta_0\in \mathcal{H}$ and let $c$ be an admissible choice of levels dependent on $\gamma_0$ and $\Pi'$. Let $\Pi=\Phi\Pi'$ and $\Gamma'=\Phi(\Theta')$.
\end{theorem}


\begin{comment}
Define
$$T_c(\theta) := \{x \in \mathcal{X}: \theta(x) = c, |(\nabla \theta)(x)| = 0\}.$$
Define the admissible level set functions
$$H^{s}_{\dagger} = \{\theta \in H^{s}(\mathcal{X}): T_{c_1}(\theta) = \emptyset, \hdots, T_{c_\mathcal{N}}(\theta) = \emptyset \},\quad s\geq 1+n/2$$
$$\Pi'(H_\dagger^{s})=1$$
\begin{proposition}
    Let $\theta_1,\theta_2\in H^{s}_{\dagger}$. If $\|\theta_1-\theta_2\|_{L^\infty(\mathcal{X})}$ is small enough, then
    \begin{equation}
        \|\Phi(\theta_1)-\Phi(\theta_2)\|_{L^2(D)} \leq C \|\theta_1-\theta_2\|_{L^\infty(\mathcal{X})}^{1/2},
    \end{equation}
    for some constant $C>0$.
\end{proposition}
\begin{proof}
    Let $\theta_\delta = \theta_2-\theta_1$ with $\|\theta_\delta\|_{\infty} < \delta$. As in \cite{igelsias2016} for $\delta$ small enough
   $$ \|\Phi(\theta_1)-\Phi(\theta_2)\|_{L^2(D)}^2 \leq \sum_{i=1}^{\mathcal{N}-1} |A_{i,\delta}| + \sum_{i=2}^{\mathcal{N}} |B_{i-1,\delta}|,$$
   where
   $$A_{i,\delta} = \{x\in \mathcal{X} : c_i \leq \theta_1(x) < c_i - \theta_\delta(x)\}$$
   $$B_{i-1,\delta} = \{x\in \mathcal{X} : c_{i-1}-\theta_\delta(x)\leq \theta_1(x) < c_{i-1}\}$$
   Clearly, it suffices to show
   $$|V_\delta|\leq C\delta \quad \text{for} \quad V_\delta:=\{x\in \mathcal{X}: |\theta_1(x)-c_i|\leq\delta\}.$$
   The inverse function theorem implies that any point $x_0\in \theta^{-1}(c_i)$ has a neighborhood $N_{x_0}$ that is a diffeomorphic image $\varphi_{x_0}(Q_{\delta_{x_0}})$ of a box
   $$Q_{\delta_{x_0}} = \{(s,t):|s|\leq \delta_{x_0}, |t|\leq \delta_{x_0}\}, \quad 0<\delta_{x_0}<1$$
    such that
    $$\theta_1(\varphi_{x_0}(s,t)) = s|(\nabla\theta_1)(x_0)|+c_i$$
    (one should find the inverse of $g(x_1,x_2)=(\frac{\theta_1(x_1,x_2)-c_i}{|\nabla\theta_1(x_0)|},x_2)$ in a neighborhood of $x_0$). Note we have a $C^1$ parametrization of a local closed neighborhood of $V_\delta$
    $$V_{\delta}\cap N_{x_0}=\{\varphi_{x_0}(s,t): |s|\leq \frac{\delta}{|\nabla\theta_1(x_0)|},|t|\leq \delta_{x_0}\},$$
    for $\delta$ small enough. 
    $$|V_{\delta}\cap N_{x_0}| = \int_{|s|\leq C(x_0,\theta_1) \delta} \int_{|t|\leq \delta_{x_0}} |J\varphi_{x_0}(s,t)| \, ds \, dt \leq C(x_0,\theta_1) \delta,$$
    since $\varphi$ is a $C^1$ function on a compact domain. Let $\cup_{x_0\in \mathcal{I}}$ be a cover of $\theta_1^{-1}(c_i)$ for some finite set $\mathcal{I}\subset \theta_1^{-1}(c_i)$. Take $V_\delta \subset \cup_{x_0\in\mathcal{I}}N_{x_0}$.
\end{proof}
\end{comment}







Let $r(\varepsilon)\geq 0$ satisfy $r(\varepsilon)\leq \varepsilon^{1-a}$ for some $0<a<1$. Further, let $\Gamma_\varepsilon\subset \Gamma$ be a sequence of Borel sets such that for all $0<\varepsilon<\varepsilon_0$
	\begin{equation}\label{eq:metric_ent}
		\log N(\Gamma_\varepsilon,d_\mathcal{G},r(\varepsilon)) \leq C_0 \left(\frac{r(\varepsilon)}{\varepsilon} \right)^2
	\end{equation}	
	for some $C_0>0$ and $\sup_{\gamma \in \Gamma_\varepsilon}\|\mathcal{G}(\gamma)\|_{\mathcal{Y}}\leq U$ for some $U>0$. Then for any $\kappa>0$, there exists statistical tests (i.e. $\{0,1\}$-valued measurable functions of the data) $\Psi_\varepsilon : \mathcal{Y}_w \rightarrow \{0,1\}$ for which
\begin{equation}
		\lim_{\varepsilon\rightarrow 0} E_{\varepsilon }^{\gamma_0} (\Psi_{\varepsilon})= 0 \quad \text{and} \quad \sup_{\gamma\in \Gamma_\varepsilon : h(p_{\varepsilon }^{\gamma_0}, p_{\varepsilon }^{\gamma})>mr(\varepsilon)/\varepsilon } E_{\varepsilon }^\gamma(1-\Psi_{\varepsilon})\leq e^{-\kappa (r(\varepsilon)/\varepsilon)^2}
\end{equation}	
with $m=m(\varepsilon_0,\kappa,C_0)$.
% Now two strategies whether it is uniform continuity or local continuity tailored towards pde solutions
\subsection{Local continuity}
 The following condition we should see as an alternative to the above condition.
\begin{condition}[Locally continuous $\Phi$]\label{cond:non-uniform}
    For $\theta_0,\theta \in \mathcal{S}_{s}(M)$ and $\|\theta_1-\theta_2\|_{L^\infty(\mathcal{X})}$ small enough, we have
    \begin{equation}\label{eq:paramcont2}
        \|\Phi(\theta)-\Phi(\theta_0)\|_{L^2(D)}\leq C \|\theta-\theta_0\|^\zeta_{L^\infty(\mathcal{X})}.
    \end{equation}
    for some constant $C=C(\theta_0)$. In addition,
    \begin{equation}\label{eq:regularsamples2}
       \Phi(\theta) \in \mathcal{T}_{t,q}(M'),
    \end{equation}
    for some uniform constant $M'>0$. If $\beta = 0$, then for any $\gamma \in \mathcal{T}_{t,q}(M'),$
    $$\|\mathcal{G}(\gamma)\|_{t} \leq M'',$$
    $t>0$.
\end{condition}









%%%% 

\newpage
with respect to $d_{\mathcal{G}}$ in the sense that
    \begin{equation}
        \log N(\Gamma',d_{\mathcal{G}},r_\varepsilon) \leq C\left(\frac{r_\varepsilon}{\varepsilon}\right)^2, \quad C>0.
    \end{equation}
Define the covering number $N(\Gamma,d_{\mathcal{G}},r_\varepsilon)$ as
$$N(\Gamma,d_{\mathcal{G}},r_\varepsilon) := \min \{n: \exists \gamma_1,\hdots,\gamma_n\in \Gamma \text{ st. } \Gamma \subset \cup_{i=1}^n B_{\mathcal{G}}(\gamma_i,r_\varepsilon)\}.$$
% Introduce \Phi again, \Phi(\Theta)\subset H^\beta. \Theta = H^beta, beta > n/2. 
% \|G(\gamma)-G(\gamma_0)\| \leq C \|\gamma-\gamma_0\|_2
% \|\Phi
% what adaptations do we need
% form of prior
% regularization sets
% argue why conditions hold
\begin{theorem}\label{thm:postcontparam}
    Suppose $\Phi$ satisfies Condition and $\mathcal{G}$ satisfies Condition . Let $\Pi'$ be a 
\end{theorem}
\subsection{Choice of base prior}
\begin{condition}[Base prior $\Pi'$]\label{cond:prior} % real-valued
	Let $\Pi''$ be a centred Gaussian probability measure on $H^\alpha(\mathcal{X})$ with $\Pi''(H^{\alpha}(\mathcal{X}))=1$. Let $\delta>\alpha>n/2$. Let the Cameron-Martin space $(\mathcal{H},\|\cdot\|_{\mathcal{H}})$ of $\Pi''$ be continuously embedded into $H^{\delta}(\mathcal{X})$. Define the prior $\Pi'=\Pi_{\varepsilon}'$ in $\Theta$ as the distribution of
$$\theta = \theta_{\varepsilon} = \varepsilon^\tau \theta'', \quad \theta'' \sim \Pi''.$$
with
$$\tau:=\frac{n}{n+2\zeta\eta \alpha}\leq 1.$$
\end{condition}



\subsection{Level-set parametrization}
\label{sec:level-set}
In this section we consider the well-known level-set parametrization of piecewise constant functions. This parametrization serves as an example for which we only have a local continuity result for the deterministic case, see Example \ref{example:nonuniform}. Even this result requires a strict subset of the usual norm-bounded Sobolev functions in $\Theta'$. 
% local continuity result
% counter example to uniform continuity
To construct the level-set parametrization take constants $c=\{c_i\}_{i=1}^{\mathcal{N}}$ satisfying 
$$-\infty = c_0 < c_1 <\hdots < c_\mathcal{N} = \infty$$
for some $\mathcal{N}\in \mathbb{N}$. Given $\theta: D\rightarrow \mathbb{R}$ define
$$A_i(\theta) :=\{x\in D: c_{i-1} \leq \theta(x) < c_i \}, \quad i=1,\hdots,\mathcal{N},$$
so that $\overline{D}=\cup_{i=1}^\mathcal{N} \overline{D}_i$ and $D_i \cap D_j = \emptyset$ for $i\neq j$. Constructing $\Theta'$ is made difficult by the fact that we in general have no uniform $C^1$ norm bound on the local graph representation of $\partial A_i(\theta)$ for $\theta \in C^1(D)$. This would require a lower bound on $|\nabla \theta|$ near $\{x\in \mathcal{D}:\theta(x) = c_i, i = 1,\hdots, \mathcal{N}\}$ as can be seen from the implicit function theorem. 
Define
$$T_c(\theta) := \{x \in D: \theta(x) = c, |(\nabla \theta)(x)| = 0\}.$$
Define the admissible level set functions
$$H^{s}_{\dagger}(D) = \{\theta \in H^{s}(D): T_{c_1}(\theta) = \emptyset, \hdots, T_{c_\mathcal{N}}(\theta) = \emptyset \},\quad s\geq 1+n/2$$
\begin{lemma}
    Let $\theta_0,\theta\in H^{s}_{\dagger}(D)$. If $\|\theta-\theta_0\|_{L^\infty(D)}<\delta_0$ for $\delta_0$ dependent on $\theta_0$, $c$ and $ \mathcal{N}$, then
    \begin{equation}
        \|\Phi(\theta)-\Phi(\theta_0)\|_{L^2(D)} \leq C \|\theta-\theta_0\|_{L^\infty(D)}^{1/2},
    \end{equation}
    for some constant $C>0$ dependent only on $D$, $c$, $\theta_0$ and $\mathcal{N}$.
\end{lemma}
\begin{proof}
    Let $\theta_\delta = \theta-\theta_0$ with $\|\theta_\delta\|_{\infty} < \delta_0$. As in \cite{igelsias2016} for $\delta_0< \max_{i=1,\hdots,\mathcal{N}}|c_{i}-c_{i-1}|$, then
   $$ \|\Phi(\theta)-\Phi(\theta_0)\|_{L^2(D)}^2 \leq \sum_{i=1}^{\mathcal{N}-1} |\mathcal{A}_{i,\delta}| + \sum_{i=2}^{\mathcal{N}} |\mathcal{B}_{i-1,\delta}|,$$
   where
   $$\mathcal{A}_{i,\delta} = \{x\in D : c_i \leq \theta_0(x) < c_i - \theta_\delta(x)\}$$
   $$\mathcal{B}_{i-1,\delta} = \{x\in D : c_{i-1}-\theta_\delta(x)\leq \theta_0(x) < c_{i-1}\}$$
   Clearly, it suffices to show that for any $i=1,\hdots,\mathcal{N}$
   \begin{equation}\label{eq:vd-condition}
       |V_\delta|\leq C\delta \quad \text{for} \quad V_\delta:=\{x\in D: |\theta_0(x)-c_i|\leq\delta\}.
   \end{equation}
   The inverse function theorem implies that any point $x_0\in \theta^{-1}(c_i)$ has a neighborhood $N_{x_0}$ that is a diffeomorphic image $\varphi_{x_0}(Q_{\delta_{x_0}})$ of a box
   $$Q_{\delta_{x_0}} = \{(s,t):|s|\leq \delta_{x_0}, |t|\leq \delta_{x_0}\}, \quad 0<\delta_{x_0}<1$$
    such that
    $$\theta_0(\varphi_{x_0}(s,t)) = s|(\nabla\theta_0)(x_0)|+c_i$$
    (one should find the inverse of $g(x_1,x_2)=(\frac{\theta_0(x_1,x_2)-c_i}{|\nabla\theta_0(x_0)|},x_2)$ in a neighborhood of $x_0$). Note we have a $C^1$ parametrization of a local closed neighborhood of $V_\delta$
    $$V_{\delta}\cap N_{x_0}=\{\varphi_{x_0}(s,t): |s|\leq \frac{\delta}{|\nabla\theta_0(x_0)|},|t|\leq \delta_{x_0}\},$$
    for all $\delta \leq |\nabla \theta_0(x_0)|\delta_{x_0}$. 
    $$|V_{\delta}\cap N_{x_0}| = \int_{|s|\leq C(x_0,\theta_0) \delta} \int_{|t|\leq \delta_{x_0}} |J\varphi_{x_0}(s,t)| \, ds \, dt \leq C(x_0,\theta_0) \delta,$$
    since the continuous function $J\varphi$ is integrated on a compact domain. Note $\cup_{x_0\in \mathcal{I}}N_{x_0}$ is an open cover of $\theta_0^{-1}(c_i)$ for some finite set $\mathcal{I}\subset \theta_0^{-1}(c_i)$ depending on $D$ and $\theta_0$. Take $\delta$ such that $V_\delta \subset \cup_{x_0\in\mathcal{I}}N_{x_0}$. Then,
    \begin{align}
        |V_\delta| &\leq \sum_{x_0\in \mathcal{I}} |V_\delta \cap N_{x_0}|\leq C(\theta_0,\mathcal{I})\delta.
    \end{align}
    This is true for any $i=1,\hdots,\mathcal{N}$ for which the estimate is only updated by a new constant.
\end{proof}
There is no uniform continuous result for the above setting, as we have a simple counter-example. 
\begin{example}\label{example:nonuniform}
    Let $D=(-\frac{1}{2},\frac{1}{2})$, $\mathcal{N}=2$, $c_1=0$, $\kappa_1=1$ and $\kappa_2=2$. Take $\theta_n = \frac{1}{n}+x^{2n}$ and $\theta_n'=-\theta_n$. It is clear that $\theta_n,\theta_n' \in H^s_\dagger(D)$ for all $n \in \mathbb{N}$ and $s\in \mathbb{R}$, and that for $n$ large enough
    $$\|\theta_n-\theta_n'\|_{C^k(D)} \leq 2\|n^{-1}\|_{C^k(D)} + 2\|x^{2n}\|_{C^k(D)} \leq C(n^{-1}+2^{-2n}).$$
    However $\Phi(\theta_n)=2$ and $\Phi(\theta_n')=1$ so that $\|\Phi(\theta_n)-\Phi(\theta_n')\|_{L^2(D)}=1$ for all $n\in \mathbb{N}$.
\end{example}
The problem is that we in general do not have a lower bound on the length of the gradient of $\theta\in H^s_\dagger(D)$. One possible remedy is to consider $\theta$ in a smaller set that is given enough mass under the Gaussian prior. It seems a condition like \eqref{eq:vd-condition} is almost (but not quite) probable enough for samples of $\Pi'$, as in \eqref{eq:scaled-prior}, in the sense of Condition \ref{cond:1.2}, using Kac-Rice type formulas for the expected excursion area, see \cite{adler2007}. Sufficient for this work is to consider the set $\Gamma'$ as
\begin{equation}\label{eq:Thetaprimelevel}
    \Gamma' = \Phi(\Theta'), \quad \Phi' = \mathcal{S}_\beta(M) \cap H^\beta_\dagger(M),
\end{equation}
and a prior $\Pi$ in $L^2_\Lambda(D)$ on the form $\Pi=\Phi\Pi'$ where $\Pi'$ is the distribution of \eqref{eq:scaled-prior} for $\beta>2+n/2$ and such that $\{\theta''(x): x\in \mathcal{X}\}$ is stationary for $\theta''\sim \Pi''$. 
\begin{theorem}
    Let $\Gamma = \Phi(H^{\alpha}(D))$, $\alpha>1+n/2$ and suppose Condition \ref{cond:forward-map} is satisfied for $\Theta'$ in \eqref{eq:Thetaprimelevel}. Define $\Pi$ as above for $\beta>2+n/2$ and let 
    $$\gamma_0 = \Phi(\theta_0),$$
    $\theta_0\in \mathcal{H}$. If $\Pi(\cdot|Y)$ is the corresponding sequence of posterior distributions arising for the model \eqref{eq:obs}. Then
    $$\Pi(\gamma:\|\gamma-\gamma_0\|_{L^2(D)}\leq f(C_0r_\varepsilon)|Y)\rightarrow 1 \quad \text{ in $P_{\varepsilon}^{\gamma_0}$-probability},$$
    where $r_\varepsilon=\varepsilon^{1-a}$ with
    $$a>\max\left\{\frac{n}{\eta \beta + n},\frac{1}{1+t\tau/2}\right\}.$$
    \begin{proof}
        It is well-known that under the prior assumptions $(\theta(x),\partial_1\theta(x),\hdots,\partial_2\theta(x))$ is a centered Gaussian vector with a constant non-degenerate covariance matrix (dependent on $\varepsilon$) for each $x\in D$, see also Exercise 6.2 \cite{azais2009}. Then by \cite[Proposition 6.12]{azais2009}
        $$\Pi'(H^\beta_\dagger(D)) = 1,$$
        for each $\varepsilon>0$. Since 
        $$H^\alpha(D)\setminus \Theta' = (H^\alpha(D) \cap \mathcal{S}_\beta(M)^c) \cup (H^\alpha(D) \cap H^\beta_\dagger(M)^c),$$
        it follows that
        $$\Pi'(H^\alpha(D)\setminus \Theta')\leq \Pi'(H^\alpha(D)\setminus \mathcal{S}_\beta(M)).$$
        Then by Lemma \ref{lemma:3.1}, Condition \ref{cond:1.2} is satisfied. The proof proceeds as in Theorem \ref{thm:3.6}.
    \end{proof}
\end{theorem}


% Proposition 6.12
% prior
% prior mass

==> old-files/old-sec-2.tex <==
We observe $\gamma \in \Gamma$ indirectly from noisy measurements. This is modelled by the (nonlinear) continuous forward map $\mathcal{G}:L^2_\Lambda(D)\rightarrow \mathcal{Y}$ for a real separable Hilbert space $(\mathcal{Y},\langle \cdot,\cdot \rangle)$, as the following observation
\label{section:2}
\begin{equation}\label{eq:obs}
    Y = \mathcal{G}(\gamma) + \varepsilon \xi,
\end{equation}
where $\varepsilon>0$ is the noise level and $\xi$ is 'white noise' in $\mathcal{Y}$, which we define as follows. We follow [Nickl, Huang] and introduce an orthonormal basis $\{e_n\}_{n=1}^\infty$ of $\mathcal{Y}$ and remark that the white noise expansion
\begin{equation}\label{eq:KLexp}
    \xi = \sum_{n=1}^\infty \xi_n e_n, \quad \xi_n \stackrel{i.i.d.}{\sim} N(0,1),
\end{equation}
is almost surely not an element of $\mathcal{Y}$. However, it is an element of the larger separable Hilbert space $\mathcal{Y}_{-}$, the closure of $\mathcal{Y}$ with respect to the norm $\|\cdot\|_{-} = \|K\cdot\|$, where $K:\mathcal{Y}\rightarrow \mathcal{Y}$ is the operator satisfying 
$$Ke_n=\lambda_n e_n, \qquad \sum_{n=1}^\infty \lambda_n^2<\infty, \quad \lambda_n>0.$$ 
Indeed, using Fubini's theorem,
$$\mathbb{E}[\|\xi\|_{-}^2] = \mathbb{E}\left [\sum_{n=1}^\infty \lambda_n^2\xi_n^2 \right] = \sum_{n=1}^\infty \lambda_n^2 < \infty,$$
since $\mathbb{E}[\xi_1^2]=1$.
It is clear that $\xi\sim N(0,K^2)$ in $\mathcal{Y}_{-}$ with trace-class covariance $K^2$ and that \eqref{eq:KLexp} is its Karhunen-Loeve expansion. 

We offer the following weak form of \eqref{eq:obs}, as is typically used in white noise models, see for example \cite{abraham2019,nickl2020}. Let $\mathcal{Y}_{+}$ be the domain of $K^{-1}$ endowed with $\langle \cdot,\cdot \rangle_{+} = \langle K^{-1}\cdot,K^{-1}\cdot \rangle$, i.e.
$$\mathcal{Y}_+ = \left\{\sum_{n=1}^\infty g_n e_n : \sum_{n=1}^\infty \lambda_n^{-2}g_n^2 < \infty \right\}.$$
It is easy to see that $(\mathcal{Y}_{+})^{*} = \mathcal{Y}_{-}$ with the dual pairing of $f\in \mathcal{Y}_{-}$ and $g\in \mathcal{Y}_{+}$ defined by
$$(f,g) = \sum_{n=1}^\infty f_n g_n, \quad \text{for} \quad f = \sum_{n=1}^\infty f_n e_n, \quad g = \sum_{n=1}^\infty g_ne_n,$$
making $\mathcal{Y}_{+}\subset \mathcal{Y} \subset \mathcal{Y}_{-},$ a Gel'fand triplet. 
%For further use below we denote $\mathcal{Y}_t$ the domain of $K^{-t/2}$ endowed with
%\begin{equation}\label{eq:tnorm}
%    \|\cdot\|_{t} := \|K^{-\frac{t}{2}}\cdot\|.
%\end{equation}
Note if one takes $\mathcal{Y}=L^2(D)$ and a suitable realization $K=(1-\Delta)^{-1}$, one can think of $\mathcal{Y}_+$ as the usual Sobolev space $H^2(D)$. 

Let $W(g)(\omega) = (\xi(\omega),g)$. By a standard argument $W(g)$ is a Gaussian random variable, in fact, for any $N\in \mathbb{N}$,
\begin{equation}\label{eq:whitenoiseproc}
    (W(g_1),\hdots,W(g_N)) \sim N(0,C),
\end{equation}
where 
$$C_{ij} = \langle g_i, g_j \rangle, \quad 1\leq i,j\leq N, \quad \text{ for } \quad g_i \in \mathcal{Y}_{+}.$$
Hence, the linear bounded map $g\mapsto W(g)$ from $\mathcal{Y}_{+}$ to $L^2(\Omega,\mathrm{Pr})$ extends to a linear isometry $W:\mathcal{Y}\rightarrow L^2(\Omega,\mathrm{Pr})$ satisfying \eqref{eq:whitenoiseproc}, which is a white noise process on $\mathcal{Y}$, see for example [Nickl Gine]. Identifying $Y$ with the corresponding extension $Y:\mathcal{Y}\rightarrow L^2(\Omega,\mathrm{Pr})$ (where we abuse notation), we arrive at the weak form of \eqref{eq:obs},
\begin{equation}\label{eq:obsprocess}
    Y(y) = \langle \mathcal{G}(\gamma), y \rangle + \varepsilon W(y), \quad y\in \mathcal{Y}.
\end{equation}
One can think of \eqref{eq:obs}, as observing a trajectory of \eqref{eq:obsprocess}. We denote the distributions of $\varepsilon\xi$ and $Y$ in $\mathcal{Y}_{-}$  by $P_\varepsilon$ and $P_\varepsilon^\gamma$ respectively. 

The posterior distribution is obtained from a probability density for the data-generating distribution $P_\varepsilon^\gamma$ and a prior distribution $\Pi$ on $L^2_\Lambda(D)$, which we equip with its Borel $\sigma$-algebra ($L^2_\Lambda(D)$ is a standard Borel space since it is a closed (Borel) subset of $L^2(D)$, which is indeed a separable Banach space). As this setting does not allow Lebesgue probability densities, instead, we express the densities of $P_\varepsilon^\gamma$ with respect to a common dominating measure. The Cameron-Martin theorem states that
$$P_\varepsilon^\gamma \ll P_\varepsilon$$
if $\mathcal{G}(\gamma)$ belongs to the so-called Cameron-Martin space of $P_\varepsilon$, see for example [Hairer]. In this Hilbert space setting, the Cameron-Martin space of $P_\varepsilon=N(0,K)$ is $K^{1/2}(\mathcal{Y}_{-})=\mathcal{Y}$, which contains $\mathcal{G}(\gamma)$ for all $\gamma\in L^2_\Lambda(D)$ by assumption. Further, the theorem gives the density of $P_\varepsilon^\gamma$ with respect to $P_\varepsilon$ as
\begin{equation}
    \frac{dP_{\varepsilon}^\gamma}{dP_\varepsilon}(Y) = \exp \left (\frac{1}{\varepsilon^2}Y(\mathcal{G}(\gamma))-\frac{1}{2\varepsilon^2}\|\mathcal{G}(\gamma)\|^2 \right),
\end{equation}
here evaluated in $Y$. We denote $p_\varepsilon^\gamma:=\frac{dP_{\varepsilon}^\gamma}{dP_\varepsilon}$ and call $\gamma\mapsto p_{\varepsilon}^{\gamma}(Y(\omega))$ for some $\omega\in\Omega$, the likelihood function. We argue as in [Nickl, 18] by continuity of $\gamma \mapsto \mathcal{G}(\gamma)$ that $(\gamma,\omega) \mapsto p_{\varepsilon }^\gamma(Y(\omega))$ is $\mathcal{B}(L^2_\Lambda(D))\times \mathcal{F}$-measurable.

Bayes' rule [ghoshal or pollard] gives the posterior distribution as a measure in $\Gamma$ as,
\begin{align}\label{eq:posteriorL2}
	\Pi(B|Y) = \frac{\int_B p_{\varepsilon }^\gamma(Y)\, \Pi(d\gamma)}{\int p_{\varepsilon }^\gamma(Y)\, \Pi(d\gamma)}, \quad B\subset \mathcal{B}(L^2_\Lambda(D)).
\end{align}
This is a so-called regular conditional distribution in the sense that $B\mapsto \Pi(B|Y(\omega))$ is a measure for every $\omega \in \Omega$ and $\omega \mapsto \Pi(B|Y(\omega))$ is measurable for every $B \in \mathcal{B}(L^2_\Lambda(D))$ and in fact a $[0,1]$-valued random variable. 
\begin{remark}
	If $\mathcal{Y}$ is a finite-dimensional Hilbert space, we have that
\begin{align}
	\Pi(B|Y) &= \frac{1}{Z}\int_{B} \exp\left (\frac{1}{\varepsilon^2}\langle Y, \mathcal{G}(\gamma) \rangle - \frac{1}{2\varepsilon^2}\|\mathcal{G}(\gamma)\|^2 \right) \, \Pi(d\gamma),\\
	&= \frac{1}{Z} \int_{B} \exp\left (-\frac{1}{2\varepsilon^2}\|\mathcal{G}(\gamma)-Y\|^2 \right) \, \Pi(d\gamma).
\end{align}
With this more common form it is easier to see that $\Pi(\cdot|Y)$ gives mass to the sets that are favored by $\Pi$ and give data close to the observed. 
\end{remark}
Note that $\Pi(\cdot|Y)$ tacitly depends on $\varepsilon$. We also recall that for any measurable $f: (\mathcal{Y}_{-},\mathcal{B}(\mathcal{Y}_{-}))\rightarrow (\mathbb{R},\mathcal{B}(\mathbb{R}))$
$$f(Y) \rightarrow 1 \quad  \text{ in $P_{\varepsilon}^{\gamma_0}$-probability}$$
with rate $r_{\varepsilon}$ as $\varepsilon \rightarrow 0$, means that
\begin{equation}\label{eq:convergenceinprob}
P_{\varepsilon}^{\gamma_0}(y \in \mathcal{Y}_{-}: |f(y)-1| \leq Cr_\varepsilon) \rightarrow 1,
\end{equation}
as $\varepsilon\rightarrow 0$ for some constant $C>0$.

==> old-files/post-cont-theorem.tex <==
\begin{lemma}\label{lemma2}
	Define the event
	$$A_\varepsilon = \left \{y\in \mathcal{Y}_-:\int_{\Gamma} (p^\gamma_{\varepsilon }/p^{\gamma_0}_{\varepsilon })(y) \, \Pi(d\gamma) \geq \Pi(B_{\mathcal{G}}(\gamma_0,r_\varepsilon)) e^{-2(r(\varepsilon)/\varepsilon)^2}\right \}$$
	Then $P_{\varepsilon }^{\gamma_0}(A_\varepsilon^c) \leq (r_\varepsilon/\varepsilon)^{-1}$.
\end{lemma}
\begin{proof}
    
\end{proof}
The interpretation is that data that gives rise to an exponentially decaying posterior denominator are given little mass by $P_{\varepsilon }^{\gamma_0}$, that is if the prior gives sufficiently mass to the neighborhoods $B_{\mathcal{G}}(\gamma_0,r_\varepsilon)$. 
%%%% Proof of Theorem 2.8 %%%%
\begin{proof}[Proof of Theorem \ref{thm:contr}]
Let
	$$\widetilde{\Gamma}_\varepsilon := B_{\mathcal{G}}(\gamma_0,C_0r_\varepsilon) \cap \Gamma'.$$
 Rewriting \eqref{eq:convergenceinprob} the property \eqref{eq:postcontrforward} holds with rate $e^{-b(r_\varepsilon/\varepsilon)^2}$ for some $b>0$ if
    $$P_n^{\gamma_0}\left(
    \Pi[\widetilde{\Gamma}_{\varepsilon} | Y]< 1-Ce^{-b(r_\varepsilon/\varepsilon)^2} \right) \rightarrow 0.$$
	%We aim to show the $P_n^{\gamma_0}$-convergence property of $\Pi_\varepsilon(\widetilde{\Gamma}_{\varepsilon}|Y)$ and use the lower bound \eqref{eq:hellequiv} permitted by condition \ref{itemd} to show the property on sets $\Gamma_\varepsilon \cap \{d_{\mathcal{G}}(\gamma,\gamma_0)\leq Cmr_\varepsilon\}$. Finally, using condition \ref{itemd} this gives \eqref{eq:postconst}.
	To show this we decompose $\mathcal{Y}_{-}$ into four events. First, consider the event
	$$\widetilde{A}_{\varepsilon}:= \left \{y\in \mathcal{Y}_-:\int_{\Gamma} (p^\gamma_{\varepsilon }/p^{\gamma_0}_{\varepsilon })(y) \, \Pi(d\gamma) \geq  e^{-(C_1+2)(r_\varepsilon/\varepsilon)^2}\right \} $$
	satisfies $A_\varepsilon \subset \widetilde{A}_\varepsilon$ implying $\widetilde{A}_\varepsilon^c \subset A^c_\varepsilon$ and hence $P_{\varepsilon }^{\gamma_0}(\widetilde{A}_\varepsilon^c)\rightarrow 0$ as $\varepsilon \rightarrow 0$. Next, the event
    $$\left \{y \in \mathcal{Y}_-: \Psi_\varepsilon(y) = 1\right\}$$
    satisfies by Condition \ref{cond:1}.\ref{cond:1.3}
    $$P_{\varepsilon }^{\gamma_0}(\Psi(Y) = 1) \rightarrow 0,$$
    as $\varepsilon \rightarrow 0$.	Then as $\varepsilon\rightarrow 0$
	\begin{align}
        P_n^{\gamma_0}&\left(\Pi[\widetilde{\Gamma}_{\varepsilon} | y]\leq 1-e^{-b(r_\varepsilon/\varepsilon)^2} \right)\\
		 &= P_n^{\gamma_0}\left(\Pi[\widetilde{\Gamma}_{\varepsilon}^c | y]\geq e^{-b(r_\varepsilon/\varepsilon)^2}\right),\\
		&= 	P_n^{\gamma_0}\left(\Pi[\widetilde{\Gamma}_\varepsilon^c | y]\geq e^{-b(r_\varepsilon/\varepsilon)^2}\cap   \widetilde{A}_\varepsilon \cap  \{\Psi_\varepsilon = 0\}\right) + o(1),\\
		&\leq P_n^{\gamma_0}\left(\int_{\widetilde{\Gamma}_{\varepsilon}^c} p^\gamma_{\varepsilon }/p^{\gamma_0}_{\varepsilon } \, \Pi(d\gamma)\geq e^{-(b+C_1+2)(r_\varepsilon/\varepsilon)^2} \cap \{\Psi_\varepsilon = 0\}\right) + o(1),\\
		&\leq P_n^{\gamma_0}\left(\int_{\widetilde{\Gamma}_{\varepsilon}^c} p^\gamma_{\varepsilon }/p^{\gamma_0}_{\varepsilon } \, \Pi(d\gamma)(1-\Psi_{\varepsilon})\geq e^{-(b+C_1+2)(r_\varepsilon/\varepsilon)^2}\right) + o(1),
		\intertext{which by Markov's inequality gives}
		&\leq e^{(b+C_1+2)(r_\varepsilon/\varepsilon)^2} E_{\varepsilon}^{\gamma_0}\left [\int_{\widetilde{\Gamma}_{\varepsilon}^c} p^\gamma_{\varepsilon }/p^{\gamma_0}_{\varepsilon } \, \Pi(d\gamma)(1-\Psi_{\varepsilon}) \right ]+o(1),
		\intertext{which by Fubini's theorem in concert with the chain rule for Radon-Nikodym derivatives gives}
		&= e^{(b+C_1+2)(r_\varepsilon/\varepsilon)^2} \int_{\widetilde{\Gamma}_{\varepsilon}^c} E_{\varepsilon}^{\gamma}(1-\Psi_{\varepsilon}) \Pi(d\gamma) +o(1),
		\intertext{which by the decomposition $\widetilde{\Gamma}_{\varepsilon}^c = \Gamma'^c \cup (B_{\mathcal{G}}(\gamma_0,C_0r_\varepsilon)^c \cap \Gamma'^c) \cup (B_{\mathcal{G}}(\gamma_0,C_0r_\varepsilon)^c \cap \Gamma')$ gives}
		&\leq e^{(b+C_1+2)(r_\varepsilon/\varepsilon)^2} \left (2\Pi_{\varepsilon}(\Gamma'^c) + \int_{B_{\mathcal{G}}(\gamma_0,C_0r_\varepsilon)^c \cap \Gamma'} E_{\varepsilon}^{\gamma}(1-\Psi_{\varepsilon}) \Pi(d\gamma)  \right )+o(1),\\
		&\lesssim e^{(b+C_1+2-C_2)(r_\varepsilon/\varepsilon)^2} + e^{(b+C_1+2-C_3)(r_\varepsilon/\varepsilon)^2} + o(1) \rightarrow 0,
	\end{align}
	where we used Condition \ref{cond:1}.\ref{cond:1.2} and \ref{cond:1}.\ref{cond:1.3}.
\end{proof}

==> old-files/riesz-rep.tex <==
 \section{White noise}
    \textcolor{red}{
\textbf{Derivation, which I don't think is necessary to include anywhere - it is basically Riesz' representation theorem}:
We should check that
\begin{enumerate}
    \item the map $f\mapsto l_f$ is well-defined ($l_f$ a bounded linear functional)
    \item $f\mapsto l_f$ is bijective
    \item $\|f\|_{-} = \|l_f\|_{(\mathcal{Y}_+)^*}$ (isometric)
\end{enumerate}
1. For any $f\in \mathcal{Y}_{-}$
$$|l_f(g)|=|(f,g)|= |\sum_{k=1}^\infty \lambda_n f_n \lambda_n^{-1}g_n|\leq \|f\|_{-}\|g\|_{+}$$
by Cauchy-Schwarz, for all $g\in \mathcal{Y}_{+}$, hence a bounded linear functional.\\
2. For injectivity assume $l_{f}=l_{f'}$, i.e.
$$l_f(g) = l_{f'}(g) \qquad \text{for all $g\in \mathcal{Y}_+$}.$$
But that is to say $(f,g) = (f',g)$, i.e. $(f-f',g)=0$ for all $g\in \mathcal{Y}_+$ by bilinearity. In particular for $g=\lambda_n e_k$
$$0=(f-f',g)=\langle f-f', \lambda_n^{-1}e_k \rangle_{-}$$
for all $n\in\mathbb{N}$. Since $\{\lambda_n^{-1} e_k\}$ is a complete orthornormal system in $\mathcal{Y}_-$ it follows $f=f'$. For surjectivity, let $l\in (\mathcal{Y}_+)^\ast$, and note our goal is to find $f \in \mathcal{Y}_-$ such that $l_f=l$. Note that since $\mathcal{Y}_+$ is a Hilbert space, we have a characterization of $(\mathcal{Y}_+)^\ast$ by Riesz representation theorem: given any $l\in (\mathcal{Y}_+)^\ast$, there exists $w \in \mathcal{Y}_+$ such that
$$l(g) = \langle g, w \rangle_{+} = \sum_{k=1}^\infty \lambda_n^{-2} g_n w_n$$
for all $g\in \mathcal{Y}_+$. Defining the element
$$f:=\sum_{k=1}^\infty \lambda_n^{-2} w_n e_k$$
we note that $l(g) = (f, g)$ and $f\in \mathcal{Y}_{-}$, since
$$\|f\|_{-}^2 = \sum_{k=1}^\infty \lambda_n^2 f_n^2 =  \sum_{k=1}^\infty \lambda_n^{-2}w_n^2 < \infty,$$
using $w\in \mathcal{Y}_+$.\\
3. By definition
$$\|l_f\|_{(\mathcal{Y}_+)^\ast} := \sup_{\|g\|_{\mathcal{Y}_+}=1}|l_f(g)| \leq \|f\|_{-}\|g\|_{+}=\|f\|_{-}$$
For the opposite direction note
\begin{align}
    \|f\|_{-}^2 = \sum_{k=1}^\infty \lambda_n^2f_n^2 &= (f, \sum_{k=1}^\infty \lambda_n^2 f_ne_k),\\
    &= |l_f(\sum_{k=1}^\infty \lambda_n^2 f_ne_k)|,\\
    &\leq \|l_f\|_{(\mathcal{Y}_+)^\ast}\|\sum_{k=1}^\infty \lambda_n^2 f_ne_k\|_{+},\\
    &=\|l_f\|_{(\mathcal{Y}_+)^\ast}\|f\|_{-},
\end{align}
hence $\|f\|_{-}\leq \|l_f\|_{(\mathcal{Y}_+)^\ast}$.
}

==> old-files/star-shaped.tex <==
\subsection{Star-shaped set parametrization}
We start by considering the parametrization for a single inclusion, i.e. $\mathcal{N}=1$. For simplicity of exposition we consider the star-shaped sets in the plane, although it is straightforward to generalize to higher dimensions. Let $\varphi:\mathbb{S}^1\rightarrow \mathbb{R}$ be a continuously differentiable function on the unit $1$-sphere, and let
\begin{equation}\label{eq:star-shaped-inclusion}
    A(\theta)=A(x,\varphi)=\{s\exp(\varphi(\vartheta))(\cos(\vartheta),\sin(\vartheta)), 0\leq s \leq 1, 0\leq \vartheta \leq 2\pi\},
\end{equation}
where $x$ is a point in $D$. We define the norm on $\Theta = D\times C^1(\mathbb{S}^1)$ as
$$\|\theta\|_{\Theta} = \|(x,\varphi)\|_{\Theta} = |x|+\|\varphi\|_{L^\infty(\mathbb{S}^1)}.$$
\begin{lemma}\label{lemma:4.1}
    Let $\theta_1,\theta_2 \in D\times C^1(\mathbb{S}^{1})$ with $\theta_i = (x_i,\varphi_i)$ and $\|\varphi_i\|_{C^1}\leq M$ for $i=1,2$. Then
    $$\|\Phi(\theta_1)-\Phi(\theta_2)\|_{L^2(D)}\leq C\|\theta_1-\theta_2\|_{\Theta}^{1/2},$$
    where $C$ only depends on $M$ and $\kappa$.
\end{lemma}
\begin{proof}
    By the triangle inequality for the symmetric difference semi-metric
    \begin{align}
        \|\Phi(\theta_1)-\Phi(\theta_2)\|^2_{L^2(D)} &\leq C|A(x_1,\varphi_1)\Delta A(x_2,\varphi_2)|,\\
        &\leq C|A(x_1,\varphi_1)\Delta A(x_1,\varphi_2)| + C|A(x_1,\varphi_2)\Delta A(x_2,\varphi_2)|.
    \end{align}
    To bound the first term, consider the map $K:[0,1]\times [0,2\pi] \rightarrow \mathbb{R}^2$,
    $$K(s,\vartheta) = [s\exp(\varphi_1(\vartheta))+(1-s)\exp(\varphi_2(\vartheta))](\cos(\vartheta),\sin(\vartheta)),$$
    which is a parametrization of the planar set $A(0,\varphi_1)\Delta A(0,\varphi_2)$. Then since,
    \begin{align}
        \frac{\partial K}{\partial s}(s,\vartheta) &= [\exp(\varphi_1(\vartheta))-\exp(\varphi_2(\vartheta))](\cos(\vartheta),\sin(\vartheta)),\\
        \left|\frac{\partial K}{\partial \vartheta}(s,\vartheta)\right| &\leq Me^M + e^M,
    \end{align}
    and hence by the classical area formula,
    \begin{align}
        |A(x_1,\varphi_1)\Delta A(x_1,\varphi_2)| &= \int_{0}^1 \int_{0}^{2\pi} |JK(s,\vartheta)| \, d\vartheta \, ds,\\
        &\leq C(M) \|\varphi_1-\varphi_2\|_{L^\infty(\mathbb{S}^1)},
    \end{align}
    where $|JK(s,\vartheta)|$ the determinant of the Jacobian of the map $K$.
    The second term is bounded using \cite{schymura2014} to the effect that
    $$|A(x_1,\varphi_2)\Delta A(x_2,\varphi_2)| \leq |x_1-x_2|\mathcal{H}^1(\partial A(x_1,\varphi_2)) \leq C(M)|x_1-x_2|.$$
\end{proof}
An attractive property of the star-shaped inclusions that arise from $C^1$ functions is that they have a $W^{s,p}$-Sobolev regularity exponent $s<1/p$. We can make this a uniform bound for functions in the right subset $\Theta'$ of $\Theta$.
\begin{lemma}\label{lemma:4.2}
    Let $\theta\in D\times C^1(\mathbb{S}^{1})$ with $\theta = (x,\varphi)$ and $\|\varphi\|_{C^1}\leq M$. Then
    $$\|\Phi(\theta)\|_{W^{s,p}(D)}\leq C(M,D,s,p),$$
    for all $1\leq p < \infty$ and $s<1/p$.
\end{lemma}
\begin{proof}
    We assume without loss of generality that $x=0$. By [Sickel99,Faraco13] we have
	$$\|\mathds{1}_{A(\theta)}\|_{W^{s,p}(\mathbb{R}^2)} \leq C(s,p,D) \left (|A(\theta)|+\int_0^{\mathrm{diam}(D)} |(\partial A(\theta))_\delta| \frac{d \delta}{\delta^{1+ps}} \right)^{1/p}.$$
    It is easy to see that $(\partial A(\theta))_\delta$ is a subset of the image of the map $K:[0,1]\times [0,2\pi] \rightarrow \mathbb{R}^2$ defined by
 $$K(s,\vartheta) = [s(1-\delta)\exp(\varphi_1(\vartheta))+(1-s)(1+\delta)\exp(\varphi_2(\vartheta))](\cos(\vartheta),\sin(\vartheta)).$$
 Using the same argument as in Lemma \ref{lemma:4.1}
 $$|(\partial A(\theta))_\delta|\leq C(M)\delta.$$
	Then for $s<1/p$,
    \begin{align}
        \int_0^{\mathrm{diam}(D)} |(\partial A(\theta))|\frac{d \delta}{\delta^{1+ps}}&\leq  C(M,D,s,p).
    \end{align}
    Using boundedness of the restriction to $D$, we arrive at the wanted property.
\end{proof}
The prior distribution $\Pi$ in $L^2_\Lambda(D)$ takes the form $\Phi\tilde\Pi'$, where $\tilde\Pi'$ is the prior distribution in $\Theta$ on the form 
\begin{equation}
    \tilde \Pi'(d\theta) = \pi(dx)\Pi'(d\varphi),
\end{equation}
where $\Pi'$ is the distribution \eqref{eq:scaled-prior} with $\beta>1+\frac{1}{2}$  and $\pi'=N(0,\varepsilon^{2a}C)$ for some positive definite covariance matrix $C$. 

\subsubsection{Multiple inclusions}
The case of multiple star-shaped inclusions is a straightforward generalization. We consider product spaces of $D\times C^1(\mathbb{S}^1)$ on the form
$$\Theta^{\mathcal{N}} := (D\times C^1(\mathbb{S}^1))^{\mathcal{N}}. $$
We consider $A_i(\theta) = A(\theta_i)$ as in \eqref{eq:star-shaped-inclusion}. We endow the product space with a product metric $\|\cdot\|_{\Theta^\mathcal{N}}$.
\begin{comment}
$$d_\infty(\theta,\theta')=\max\left\{\|\theta_1-\theta'_1\|_{\Theta},\hdots,\|\theta_\mathcal{N}-\theta_\mathcal{N}'\|_{\Theta} \right\}.$$
\end{comment}
When $\mathcal{N}>1$, $\Phi(\theta)$ may consist of multiple overlapping inclusions, which can be handled as in the following lemma. 
\begin{lemma}
    Let $\theta_i, \theta_i' \in D\times C^1(\mathbb{S}^1)$ with $\theta_i=(x_i,\varphi_i)$, $\theta_i'=(x_i',\varphi_i')$ and $\|\varphi_i\|_{C^1}\leq M$, $\|\varphi_i'\|_{C^1}\leq M$ for $i=1,\hdots,\mathcal{N}$. Then
    $$\|\Phi(\theta)-\Phi(\theta')\|_{L^2(D)}\leq C\|\theta-\theta'\|_{\Theta^{\mathcal{N}}}^{1/2},$$
    where $C$ only depends on $M$, $\max_{i=1,\hdots,\mathcal{N}} \kappa_i$ and $\mathcal{N}$.
\end{lemma}
\begin{proof}
    Using the triangle inequality and Lemma \ref{lemma:4.1},
    \begin{align}
        \|\Phi(\theta)-\Phi(\theta')\|_{L^2(D)}^2 &\leq C \left(\sum_{i=1}^{\mathcal{N}} \|\mathds{1}_{A(\theta_i)}-\mathds{1}_{A(\theta_i')}\|_{L^2(D)}\right)^2,\\
        &\leq C\left(\sum_{i=1}^{\mathcal{N}} \|\theta_i-\theta_i'\|_{\Theta}^{1/2}\right)^2,\\
        &\leq C\|\theta-\theta'\|_{\Theta^{\mathcal{N}}}. 
    \end{align}
\end{proof}
\begin{comment}
However, when $A(\theta_i)$ and $A(\theta_j)$ for $i\neq j$ are separated the following continuity result is straightforward. 
\begin{lemma}\label{lemma:4.3}
    Let $\mathcal{N}>1$ and $\theta_i, \theta_i' \in D\times C^1(\mathbb{S}^1)$ with $\theta_i=(x_i,\varphi_i)$, $\theta_i'=(x_i',\varphi_i')$ and $\|\varphi_i\|_{C^1}\leq M$, $\|\varphi_i'\|_{C^1}\leq M$ for $i=1,\hdots,\mathcal{N}$. Suppose $\mathrm{dist}(A(\theta_i),A(\theta_j))\geq \delta_0$ for all $i\neq j$, $i,j=1,\hdots,\mathcal{N}$ for some $\delta_0 > 0$. Then for $d_\infty(\theta,\theta')< \frac{\delta_0}{2}$, we have
    $$\|\Phi(\theta)-\Phi(\theta')\|_{L^2(D)}\leq Cd_\infty(\theta,\theta')^{1/2},$$
    where $C$ only depends on $M$ and $\kappa_1,\hdots,\kappa_{\mathcal{N}}$.
\end{lemma}
\begin{proof}
    When $d_\infty(\theta,\theta')<\frac{\delta_0}{2}$ it follows that $A(\theta_i)\cap A(\theta_j')=\emptyset$ and $A(\theta_i')\cap A(\theta_j')=\emptyset$ for all $i\neq j$. Assume that $y\in A(\theta_j')$. Then $d(y,A(\theta_j))<\frac{\delta_0}{2}$. In fact, the Hausdorff distance satisfies
    \begin{align}
        d_H(A(\theta_j),A(\theta_j')) &\leq d_H(A(x_j,\varphi_j),A(x_j',\varphi_j)) + d_H(A(x_j',\varphi_j),A(x_j',\varphi_j)),\\
        &\leq |x_j-x_j'| + \|\varphi_j-\varphi_j'\|_{L^\infty(\mathbb{S}^1)} = \|\theta_j-\theta_j'\|_{\Theta}.
    \end{align}
    From the triangle inequality
    \begin{align}\label{eq:firstlowbound}
        d(y,A(\theta_i)) \geq d(A(\theta_i),A(\theta_j)) - d(y,A(\theta_j)) > \frac{\delta_0}{2},
    \end{align}
    for all $i\neq j$, which implies $A(\theta_i)\cap A(\theta_j')=\emptyset$. Similarly, since $d(y,A(\theta_i))\leq d(y,A(\theta_i)') + d_H(A(\theta_i)',A(\theta_i))$,
    \begin{align}\label{eq:secondlowbound}
        d(y,A(\theta_i')) &\geq d(A(\theta_i),A(\theta_j)) - d_H(A(\theta_j),A(\theta_j')) - d(y,A(\theta_j))>0,
    \end{align}
    for all $i\neq j$, which implies $A(\theta_i')\cap A(\theta_j')=\emptyset$. Then
    $$\|\Phi(\theta)-\Phi(\theta')\|_{L^2(D)}^2 \leq \sum_{i=1}^\mathcal{N} \kappa_i |A(\theta_i)\Delta A(\theta_i')|.$$
    The result then follows from the argument in Lemma \ref{lemma:4.1}, and the fact that all norms are equivalent on $\mathbb{R}^{\mathcal{N}}$.
\end{proof}
\end{comment}
It is clear that also Lemma \ref{lemma:4.2} holds with $\|\Phi(\theta)\|_{W^{s,p}(D)}\leq C(M,D,s,p,\mathcal{N})$ for all $1\leq p<\infty$ and $s<1/p$. The natural prior distribution $\Pi$ in $L^2_\Lambda(D)$ takes the form 
\begin{equation}\label{eq:priormultiproduct}
    \Pi = \Phi\tilde\Pi', \qquad \text{where } \quad
    \tilde \Pi'(d\theta) = \pi(dx_1)\Pi'(d\varphi_1)\hdots \pi(dx_\mathcal{N})\Pi'(d\varphi_\mathcal{N}),
\end{equation}
where $\Pi'$ is the distribution \eqref{eq:scaled-prior} for $\beta > 1+\frac{1}{2}$ and $\pi'=N(0,\varepsilon^{2a}C)$ for some positive definite covariance matrix $C$. The natural generalization of $\Gamma'$ is the set
\begin{equation}\label{eq:gammaprime-multi}
    \Gamma' = \Phi(\Theta'), \quad \Theta' = (B(M)\times \mathcal{S}_s(M))^{\mathcal{N}},
\end{equation}
for $s=\beta$. Indeed, the Sobolev embedding theorem gives that each $\varphi_i\in \mathcal{S}_s(M))$ satisfies $\|\varphi_i\|_{C^1}\leq M'$.

\begin{theorem}
    Let $\Gamma = \Phi(\Theta^{\mathcal{N}})$ and suppose Condition \ref{cond:forward-map} is satisfied for $\Theta'$ in \eqref{eq:gammaprime-multi}. Define $\Pi$ as in \eqref{eq:priormultiproduct} and let 
    $$\gamma_0 = \Phi(x_1,\varphi_1,\hdots,x_\mathcal{N},\varphi_{\mathcal{N}}),$$
    with $x_i\in \mathbb{R}^2$ and $\varphi_i \in \mathcal{H}$ for all $i=1,\hdots,\mathcal{N}$.
    If $\Pi(\cdot|Y)$ is the corresponding sequence of posterior distributions arising for the model \eqref{eq:obs}. Then
    $$\Pi(\gamma:\|\gamma-\gamma_0\|_{L^2(D)}\leq f(C_0r_\varepsilon)|Y)\rightarrow 1 \quad \text{ in $P_n^{\gamma_0}$-probability},$$
    where $r_\varepsilon=\varepsilon^{1-a}$ with
    $$a\geq\frac{1}{\eta (1+\frac{1}{2}) + 1}.$$    
\end{theorem}
\begin{proof}
\begin{remark}\label{remark:onproductprior}
      Suppose $\Pi$ is on the form $\Pi=\Phi \tilde\Pi'$ where $\tilde\Pi'=\pi'\otimes \Pi'$ is a product prior on $\mathbb{R}^n\times H^\alpha(\mathcal{X})$ with $\pi'=N(0,\varepsilon^{2a}C)$ for some positive definite covariance matrix $C$, and $\Pi'$ the distribution in \eqref{eq:scaled-prior}. If Condition \ref{cond:unifcont} is satisfied for some suitable product norm on $\mathbb{R}^n\times L^\infty(\mathcal{X})$, then the previous lemma holds for the same choice of $a$. 
  \end{remark}
  \begin{remark}\label{remark:3}
    Suppose $\Theta'$ is of the form $\Theta' = B(M)\times \tilde\Theta'$ for $\tilde \Theta'\subset \mathcal{S}_s(M)$ and $B(M)$ an ball of radius $M$ in $\mathbb{R}^n$ for some $n\in \mathbb{N}$, and Condition \ref{cond:unifcont} is satisfied for some suitable product norm on $\mathbb{R}^n\times L^\infty(\mathcal{X})$, then the previous lemma also holds with the same choice of $a$. This is immediate from the fact that $N(B(M),\|\cdot\|_2,\delta)\leq C(M,n) \delta^{-n}$ and the fact that
    $$N(A\times B,d,\delta) \leq N(A,d_X,\delta)N(B,d_Y,\delta),$$
    for $A\subset X$, $B\subset Y$ and $d$ a product norm.
\end{remark}
    It is straightforward that this choice satisfies Condition \ref{cond:1.1} given Condition \ref{cond:forward-map} as in Lemma \ref{lemma:small-ball} for $C_1$ now dependent on $\mathcal{N}$. Condition \ref{cond:1.2} is satisfied for the choice

Following Remark \ref{remark:3} and \eqref{eq:coveringnumber} it is also clear that
\begin{align}
    \log N(\Theta', \|\cdot\|_{\Theta^{\mathcal{N}}},\delta) &\leq C(M,n,s,\mathcal{N}) (\mathcal{N}\log(\delta^{-n}) + \mathcal{N}\delta^{-n/s}),\\
    &\leq C(M,n,s,\mathcal{N}) \delta^{-n/s}.
\end{align}
This permits the use of Lemma \ref{lemma:tests} as in Lemma \ref{lemma:3.3}, resulting in Condition \ref{cond:1.3} being satisfied for
$$a>\frac{n}{2s\zeta\eta+n}.$$
\end{proof}
%% insert theorem here
% define prior for which beta, what should alpha be?
% define a
% posterior consistency


 
\begin{comment}
However, Condition \ref{cond:1.3} needs some care, when we only have the local continuity result \ref{lemma:4.3}.
\begin{lemma}
    Suppose Condition \ref{cond:forward-map} is satisfied for the choice of $\Theta'$ in \eqref{eq:gammaprime-multi}. Then Condition \ref{cond:1.3} is satisfied for $\Gamma'$ and 
    $$a>$$
\end{lemma}
\begin{proof}
    We bound $\log(\Gamma',\|\cdot\|_{L^2(D)},\delta)$ directly using a well-known result in [dudley]. Note equivalently to \eqref{eq:gammaprime-multi} we have
    $$\Gamma' = \{\gamma = \sum_{i=1}^{\mathcal{N}} \kappa_i \mathds{1}_{A(\theta_i)}, \theta_1\in (B(M)\times \mathcal{S}_s(M)), \hdots, \theta_{\mathcal{N}} \in (B(M)\times \mathcal{S}_s(M))\}$$
    which is a Lipschitz continuous map of the set
    $$\{$$
    
    attack directly logN of Gamma', in L2 distance.
    use dudley
\end{proof}
\end{comment}
